ZeRO-Infinity: Breaking the GPU Memory Wall for Extreme Scale Deep Learning

In the last three years, the largest dense deep learning models have grown over 1000x to reach hundreds of billions of parameters, while the GPU memory has only grown by 5x (16 GB to 80 GB). Therefore, the growth in model scale has been supported primarily though system innovations that allow large models to fit in the aggregate GPU memory of multiple GPUs. However, we are getting close to the GPU memory wall. It requires 800 NVIDIA V100 GPUs just to fit a trillion parameter model for training, and such clusters are simply out of reach for most data scientists. In addition, training models at that scale requires complex combinations of parallelism techniques that puts a big burden on the data scientists to refactor their model. In this paper we present ZeRO-Infinity, a novel heterogeneous system technology that leverages GPU, CPU, and NVMe memory to allow for unprecedented model scale on limited resources without requiring model code refactoring. At the same time it achieves excellent training throughput and scalability, unencumbered by the limited CPU or NVMe bandwidth. ZeRO-Infinity can fit models with tens and even hundreds of trillions of parameters for training on current generation GPU clusters. It can be used to fine-tune trillion parameter models on a single NVIDIA DGX-2 node, making large models more accessible. In terms of training throughput and scalability, it sustains over 25 petaflops on 512 NVIDIA V100 GPUs(40% of peak), while also demonstrating super linear scalability. An open source implementation of ZeRO-Infinity is available through DeepSpeed, a deep learning optimization library that makes distributed training easy, efficient, and effective.

==> Makefile <==
PAPER=main

all: pdf
pdf: $(PAPER).pdf

SECTIONS = \
	evaluation.tex

TEXT = $(SECTIONS) 

TEX = main.tex \
        $(TEXT)

$(PAPER).bbl: references.bib
	export TEXINPUTS=.:./latex-styles:; \
	pdflatex $(PAPER); bibtex $(PAPER); pdflatex $(PAPER); pdflatex $(PAPER)

$(PAPER).pdf: $(TEX) $(FIGS) $(PAPER).bbl
	export TEXINPUTS=.:./latex-styles:; \
	pdflatex $(PAPER); bibtex $(PAPER); pdflatex $(PAPER); pdflatex $(PAPER)

clean:
	/bin/rm -f $(PAPER).aux $(PAPER).bbl $(PAPER).blg $(PAPER).dvi \
	$(PAPER).log $(PAPER).ps $(PAPER).pdf $(PAPER).out




==> background.tex <==
\begin{comment}

In addition to parallelism based approaches to reduce the memory footprint /cite{}


\section{Background}
DL training iteratively processes data samples in steps, and each step consists of a forward propagation, followed by a backward propagation, which is followed by weight updates. To scale DL training across GPUs, each step must be parallelized due to sequential dependency across steps. Data parallelism and model parallelism are the two most prominent ways to parallelize a DL training step across multiple GPUs. 

\subsection{Data Parallel Training}

For a model that fits in GPU memory for training, data parallelism (DP) is used to scale the training to multiple GPUs. In data parallelism, model parameters are replicated on each GPU process during initialization. At each step, a mini-batch is divided evenly across all the data parallel processes, such that each process executes the forward and backward propagation on a different subset of data samples.  

At the end of the backward propagation, the gradients are averaged across all processes, using an all-reduce communication collective, which creates a copy of the averaged gradients on each data parallel process. Each process then uses the averaged gradients to compute and apply the weight updates to its copy of the model parameters. 

Note that in data parallelism, the OGP states (weight parameters, average gradients, and optimizer states) are replicated across all the data parallel processes, incurring massive redundancy.
%as each process performs weight updates to its local copy of the parameters.
\subsection{Model Parallel Training}
While model parallelism (MP) may serve other purposes such as reducing the aggregate batch size, it is primarily used to reduce the memory footprint per GPU. 

Model parallelism divides a model into multiple partitions and performs the corresponding forward and backward computation across devices, i.e., the computation for each input data sample is partitioned and executed on multiple devices.  Model parallelism can work in two ways: i) via vertical partitioning \cite{GPipe, DBLP:journals/corr/pipedream}, and ii) via horizontal partitioning \cite{DBLP:journals/corr/mesh-tensor, megatronlm}. Vertical partitioning splits the model by partitioning the total layers in the DL model across multiple GPUs, and uses  pipelined micro-batches to avoid GPU stalls. Horizontal partitioning, on the other hand, splits individual DL layers across multiple-GPUs by parallelizing the underlying computation such as matrix multiplication or element-wise operation.

While each of these techniques has their pros and cons in terms of training throughput and batch size implications, the underlying effect in terms of memory consumption is the same. Both reduces the memory footprint per GPU by partitioning the activations, model parameters, gradients, and optimizer states across multiple GPUs. 
\end{comment}

==> conclusion.tex <==
\section{Concluding Remarks}


==> figures/tables/merged_speed_table.tex <==
\begin{table}[]
\caption{Configurations for performance evaluations.}
%\vskip -0.7em
% \scriptsize
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \# DGX-2 nodes& \# params& batch/GPU&  mp & \ fp16 param & Opt State  \\ \hline %\hline
1 & 10 billion  &  8  & 1 & GPU & GPU \\ \hline
1 & 50, 100 billion  & 26, 24  & 1 & CPU & NVMe \\ \hline
1 & 0.5, 1 trillion & 8, 7 & 1 & NVMe    &  NVMe   \\ \hline
32 & 0.5, 1 trillion & 7, 5  & 4 & GPU & GPU \\ \hline
32 & 5, 10, 20 trillion& 3, 2, 1.25 & 4, 4, 8  & NVMe    &  NVMe   \\ \hline
\end{tabular}
}
\label{tab:model_perf_configs}
%\vskip -2em
\end{table}


==> figures/tables/model_config.tex <==
\begin{table}[]
\caption{Model configurations.}
%\vskip -0.7em
%\scriptsize
\centering
\begin{tabular}{|c|c|c|}
\hline
 \# params& hidden size& \# layer \\ \hline %\hline
8 billion & 8192 & 10 \\ \hline
10, 50, 100 billion  & 4096, 8192, 8192 & 50, 62, 125   \\ \hline
0.5, 1 trillion  & 18432, 25600  & 124, 128 \\ \hline
5, 10 trillion & 49152, 65536 & 174, 200 \\ \hline
20 trillion  & 90112  & 205 \\ \hline
\end{tabular}
\label{tab:model}
%\vskip -2em
\end{table}


==> figures/tables/speed_1node.tex <==
\begin{table}[]
%\vskip 1em
\caption{Configurations for 1 node evaluation.}
%\vskip -0.7em
% \scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
 \# params& batch/GPU& mp& fp16 param & Opt State  \\ \hline %\hline
10 billion  &  8  & 1 & GPU & GPU \\ \hline
50, 100 billion  & 26, 24  & 1 & CPU & NVMe \\ \hline
0.5, 1 trillion & 8, 7 & 1 & NVMe    &  NVMe   \\ \hline
\end{tabular}
\label{tab:speed_1node}
%\vskip -2em
\end{table}

==> figures/tables/speed_512gpu.tex <==
\begin{table}[]
\caption{Configurations for evaluation on 512 GPUs.}
%\vskip -0.7em
% \scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
 \# params& batch/GPU&  mp & \ fp16 param & Opt State  \\ \hline %\hline
0.5, 1 trillion & 7, 5  & 4 & GPU & GPU \\ \hline
5, 10, 20 trillion& 3, 2, 1.25 & 4, 4, 8  & NVMe    &  NVMe   \\ \hline
\end{tabular}
\label{tab:perf_512gpu}
%\vskip -2em
\end{table}

==> figures/tables/zinf_configs.tex <==

\newcommand{\myGPU}{\color{black} GPU}
\newcommand{\myCPU}{\color{purple} CPU}
\newcommand{\myNVMe}{\color{blue} NVMe}

\begin{table}[]
\caption{Device placement options and sharding strategies for ZeRO-based optimizer, gradient, and parameter states.}
%\vskip -0.7em
\small
\centering
\begin{tabular}{|c|c|c|}
\hline
 Name & 
 \begin{tabular}[c]{@{}c@{}} Optimizer + Gradients \\ (devices/sharded) \end{tabular} & 
 \begin{tabular}[c]{@{}c@{}} Parameters \\ (devices/sharded)\end{tabular}  \\ \hline
Data parallelism & [GPU] / \mycrossout & [GPU] / \mycrossout \\ \hline
ZeRO 2~\cite{zero}         & [GPU] / \mycheckmark  & [GPU] / \mycrossout   \\\hline
ZeRO-Offload~\cite{zero-offload}   & [CPU,GPU] / \mycheckmark  & [GPU] / \mycrossout   \\\hline
3D Parallelism~\cite{3dparallelism} & [GPU] / \mycheckmark  & [GPU] / \mycheckmark   \\\hline
ZeRO 3~\cite{zero}         & [GPU] / \mycheckmark  & [GPU] / \mycheckmark   \\\hline
ZeRO-Inf-CPU               & [CPU,GPU] / \mycheckmark  & [CPU,GPU] / \mycheckmark   \\\hline
ZeRO-Inf-NVMe  & [NVMe,CPU,GPU] / \mycheckmark & [NVMe,CPU,GPU] / \mycheckmark  \\ \hline
\end{tabular}
\label{tab:zero-inf-configs}
%\vskip -2em
\end{table}

%ZeRO-Inf-CPU_2  & \myCPU / \mycheckmark  & \myCPU / \mycheckmark   \\\hline
% ZeRO-Inf-NVMe & \myNVMe / \mycheckmark & \myCPU / \mycheckmark   \\ \hline
%ZeRO-Inf-NVMe_2 & \myNVMe / \mycheckmark & \myNVMe / \mycheckmark  \\ \hline
% \begin{table}[]
% \begin{tabular}{lccl}
% Name          & \multicolumn{1}{l}{State}                                           & \multicolumn{1}{l}{Location}         &  \\
% \textbf{Name} & \multicolumn{1}{l}{\textbf{Optimizer + gradients (device/sharded)}} & \textbf{Parameters (device/sharded)} &  \\
% ZeRO 2         & GPU / ✓  & GPU / -  &  \\
% ZeRO-Offload   & CPU / ✓  & GPU / -  &  \\
% 3D Parallelism & GPU / ✓  & GPU / ✓  &  \\
% ZeRO 3         & GPU / ✓  & GPU / ✓  &  \\
% ZeRO-Inf-CPU1  & CPU / ✓  & GPU / ✓  &  \\
% ZeRO-Inf-CPU2  & CPU / ✓  & CPU / ✓  &  \\
% ZeRO-Inf-NVMe1 & NVMe / ✓ & CPU / ✓  &  \\
% ZeRO-Inf-NVMe2 & NVMe / ✓ & NVMe / ✓ & 
% \end{tabular}
% \end{table}

% Name &
%   \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Optimizer + gradients \\ (device/sharded)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}Parameters \\ (device/sharded)\end{tabular} &
%   \\

% [OS+Grads,Params] locations [GPU,CPU,NVMe]

% ZeRO-2 (10B)
% ZeRO Offload (13B)
% 3D parallelism (20B) (verify)
% ZeRO Stage 3 (20B) (verify)
% ZeRO-Infinity (OS to CPU) (70B) (?)
% ZeRO-Infinity (70B) (OS+Param to CPU) (80B) (?)
% ZeRO-Infinity (OS to NVMe, params to CPU) (400B) (?)
% ZeRO-Infinity (1000B) (params to NVMe)

% ZeRO-3   OS_GPU + P_GPU
% ZeRO-3   OS_CPU + P_GPU
% ZeRO-3   OS_CPU + P_CPU
% ZeRO-Inf OS_NVMe + P_CPU
% ZeRO-Int OS_NVMe + P_NVMe



==> merged_micro_eval_figures.tex <==
\begin{figure*}
     \centering
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figures/max-model-size.PNG}
    %      \caption{max model size}
    %      \label{fig:max-model-size}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figures/memory-centric-tiling.PNG}
    %      \caption{memory-centric tiling}
    %      \label{fig:tiling-perf}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{z2-v-zinf-8B.PNG}
    %      \caption{\name vs zero-2}
    %      \label{fig:zinf-v-z2}
    %  \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/overlap-perf.PNG}
         \caption{prefetch}
         \label{fig:prefetch-perf}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ac-overhead.PNG}
         \caption{activation ckpt}
         \label{fig:activation-ckpt-perf}
     \end{subfigure}
     \begin{subfigure}[b]{0.40\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/bw-req-table.PNG}
         \caption{Bandwidth requirements on NVIDIA V100 as well as future accelerators with 10x and 100x compute for ZeRO-Infinity to remain efficient on a 512 device cluster.}
         \label{fig:zero-inf-configs}
     \end{subfigure}
        % \vspace{1em}
        \caption{main caption}
        \label{fig:merged_micro_eval}
\end{figure*}

% \begin{table}[]
% \begin{tabular}{|c|c|c|c|}
% \hline
%                           & V100 & 10x  & 100x  \\ \hline
% Total devices                    & 512  & 512  & 512   \\ \hline
% Achievable peak (pflops/device)  & 0.07 & 0.70 & 7.00  \\ \hline
% Bw requirement (GB/s per device) & 3.0  & 30.0 & 300.0 \\ \hline
% Aggregate bw (TB/s)              & 1.5  & 15.0 & 150.0 \\ \hline
% GPU-to-GPU bw (GB/s)             & 70.0 & 70.0 & 700.0 \\ \hline
% \end{tabular}
% \end{table}

%% bw req table
% \begin{table*}[]
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Device &
%   \begin{tabular}[c]{@{}c@{}}Total \\ device\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Achievable peak\\ (pflops/device)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Bw requirement\\ (GB/s per device)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Aggregate\\ bw (TB/s)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}GPU-to-GPU\\ bw (GB/s)\end{tabular} \\ \hline
% V100 & 512 & 0.07 & 3.0   & 1.5   & 70.0  \\ \hline
% 10x  & 512 & 0.70 & 30.0  & 15.0  & 70.0  \\ \hline
% 100x & 512 & 7.00 & 300.0 & 150.0 & 700.0 \\ \hline
% \end{tabular}
% \end{table*} 

\begin{figure}
  \begin{minipage}[t]{0.5\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/max-model-size.PNG}
    \captionof{figure}{\small{Max model size \vspace{1pt}}}
    \label{fig:max-model-size}
  \end{minipage}
  \quad
  \begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/z2-v-zinf-8B.PNG}
    \captionof{figure}{\small{ZeRO-Inf vs ZeRO Offload}}
  \end{minipage}
  \quad
  \begin{minipage}[t]{0.60\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/zero-inf-table.PNG}
    \small
    \captionof{figure}{\small{Device/sharding strategies}}
    \label{fig:max-model-size}
  \end{minipage}
  \quad
  \begin{minipage}[t]{0.35\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/memory-centric-tiling.PNG}
    \captionof{figure}{\small{Memory-centric tiling factors}}
  \end{minipage}
\end{figure}




% \begin{table}[]
%   \caption{Device placement options and sharding strategies for ZeRO-based optimizer, gradient, and parameter states.}
% %   \small
%   \centering
%   \begin{tabular}{|c|c|c|}
%     \hline
%     Name & \begin{tabular}[c]{@{}c@{}} Opt + Grad \\ (devices/sharded) \end{tabular} & \begin{tabular}[c]{@{}c@{}} Parameters \\ (devices/sharded)\end{tabular}  \\ \hline
%     Data parallel & [GPU] / \mycrossout & [GPU] / \mycrossout \\ \hline
%     ZeRO 2         & [GPU] / \mycheckmark  & [GPU] / \mycrossout   \\\hline
%     ZeRO-Offload   & [CPU,GPU] / \mycheckmark  & [GPU] / \mycrossout   \\\hline
%     3D Parallelism & [GPU] / \mycheckmark  & [GPU] / \mycheckmark   \\\hline
%     ZeRO 3         & [GPU] / \mycheckmark  & [GPU] / \mycheckmark   \\\hline
%     ZeRO-Inf-CPU               & [CPU,GPU] / \mycheckmark  & [CPU,GPU] / \mycheckmark   \\\hline
%     ZeRO-Inf-NVMe  & [NVMe,CPU,GPU] / \mycheckmark & [NVMe,CPU,GPU] / \mycheckmark  \\ \hline
% \end{tabular}
% \label{tab:zero-inf-configs}
% \end{table}

% \begin{figure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/max-model-size.PNG}
%         \caption{max model size}
%         \label{fig:max-model-size}
%     \end{subfigure}
     
%     \hfill
     
%     \begin{subfigure}[b]{0.32\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{figures/memory-centric-tiling.PNG}
%      \caption{memory-centric tiling}
%      \label{fig:tiling-perf}
%     \end{subfigure}

%     \hfill

%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{z2-v-zinf-8B.PNG}
%         \caption{\name vs zero-2}
%         \label{fig:zinf-v-z2}
%     \end{subfigure}

%     \hfill
    
%     \begin{subfigure}[b]{0.40\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/zero-inf-table.PNG}
%         \caption{zero-based configs}
%         \label{fig:zero-inf-configs}
%     \end{subfigure}

% \end{figure}

==> perf_tuning.tex <==
%\section{Performance tuning for massive models}
%We may have to skip this section for now

==> results.tex <==

 

 
 


==> trillion.tex <==
\section{Step Towards 1 Trillion Parameters}
The largest published models today are in the range of 10 billion parameters, which are already challenging to train.  Getting to a trillion parameters,  3-orders of magnitude larger, will inevitably happen, but the road will be full of hurdles, surprises, and innovations. While we do not claim knowing or addressing all of them, \name addresses one of the most fundamental challenges from a system perspective: the ability to fit a model of this scale on current hardware while allowing it to train with good system scalability.

\textbf{A Leap from State-of-Art}  
The largest model that the state-of-art framework, Megatron, can train with acceptable throughput is a 16 - 20B parameter model in a DGX-2 system. Scaling further by having model parallelism across multiple DGX nodes results in a significant efficiency drop due to limited internode bandwidth.  

\name vastly increases the efficiently-runnable model size.  It enables the current generation of hardware to run significantly larger models without requiring fine-grained model parallelism to go across the node boundaries.
As demonstrated in Table~\ref{tab:memory-consumption}, \name, with all optimizations turned on (P$_{os+g+p}$), could fit more than 1 \emph{Trillion} parameters on 1024 GPUs using DP only.  Alternatively, when combined with model parallelism (as shown in Table \ref{tab:largest-model}), \name could fit more than 1 \emph{Trillion} parameters on 1024 GPUs with 16-way model parallelism (within each DGX2 node) and 64-way data parallelism across nodes.  Running a model with a trillion parameters efficiently is no longer impossible!

 
%Combined with any form of model parallelism, \name enables the current generation of hardware to run significantly larger model without requiring fine-grained model parallelism to go across the node boundaries.
%As demonstrated in Table \ref{tab:largest-model}, \name, with all optimizations turned on (P$_{os+g+p}$), could fit $2$ \emph{Trillion} parameters on 1024 GPUs with 16-way model parallelism (within each DGX2 node) and 64-way data parallelism across nodes.  Running a model with a trillion parameters efficiently is no longer impossible!

%It is trivial to go larger by using model parallelism across multiple nodes, but as the authors of Megatron themselves noticed, this would result in a significant efficiency drop due to poor interconnect bandwidth across boxes. More specifically, the bisection bandwidth inside a DGX-2 box is about 2.4 TB/s while across boxes, the bi-section bandwidth drops to a meager 200 GB/sec. Due to this drop in bandwidth, scaling a large model past a single node via model-parallelism is not possible. 

%\textbf{Combining \name with Model Parallelism} As discussed in Sec.\ref{sec:backgroud}, Model Parallelism is used in conjunction with Data Parallelism, to train large models that would other wise not fit in a single GPU. As such, \name can be combined with any form of model parallelism, to enables the current generation hardware to run significantly larger model with the same model parallelism degree without requiring to go across node boundaries. Table.~\ref{tab:largest-model}, shows the largest model that can be run for a given degree of model parallelism and data parallelism.  In the table the baseline columns represents the current state-of-art approach. Note that with 16-way model parallelism, in theory (without any activation and other memory overheads) we can at most run a 32B parameter model with the baseline, while \name, with its various memory optimizations turned on, can fit 121 Billion, 230 Billion and 2 Trillion using $P_{os}$, $P_{os+g}$, P$_{os+g+p}$, respectively. 

\textbf{Compute Power Gap} Training a trillion parameter model end-to-end within an acceptable time range, however, could still require a significant amount of compute power, which is lacking in today's AI clusters.

%Indeed, we can fit a model with over a trillion parameters using 16-way model parallelism, and 64-way data parallelism, and train it effectively since we are neither crossing the node boundary, or increasing the inter-node data-movement significantly (as discussed in Sec. ~\ref{communication-volume}). However, we would like to caution the reader, that training such a model in a reasonable time would still require significant amount of GPU resources. 

To understand the resource requirement, we present a brief comparison with Bert-Large. Bert-Large can be trained in $67$ minutes on a $1024$ GPU DGX-2H cluster \cite{nvidia-bert-training-with-gpus}. A 1 Trillion Parameter model can easily contain $3000$x (1 trillion / 330 million) more computation than a Bert-Large model for a data sample.  Even if we assume the same sequence length and the total number of samples required to train the model, training a 1T model would take 140 days, assuming the same hardware and similar computational efficiency.  In practice, both data samples and sequence length are likely to increase with the increased model size requiring over a year to train.  It would require an exa-flop system to train a 1T parameter model in a reasonable time. However, when such compute capacity becomes available, we hope \name will provide the system technology to run the 1T models efficiently. 


%\textbf{Immediate Impact} While 1T parameter model requires exa-flop supercomputers, a 100B parameter model may be trained in a few weeks on a 1024 GPU system which already exists, once again assuming same sequence length and data size, and similar computational efficiency. As such, for our first release of \name, we implement $P_{os}$, which enables us to train a 100B parameter model with a 16-way model parallelism. 

%Next we discuss this implementation and demonstrate its effectiveness.

\begin{comment}


Until such a system is available, our model 

Based on our memory consumption models described in Sec.~\ref{memory-consumption-models}, 32B parameter model is the largest possible model that we fit with 16-way model parallelism. In practise, we find can fit 20B parameters using Megatron.



Going beyond a 16B parameter model would require extending model parallelism across a single node,  
The current state-of-art framework on large model training can, which can fit a 16B parameter model in a 16-GPU system such as the DGX-2 box. The authors of Megatron themselves state that currently it is imporssible to 



and in out opinion the first major road block is the ability to fit a model of this size and train it with a reasonable at a reasonable throughput. 

a major one is the ability to fit a model of this size 


With all the aforementioned memory optimizations, the memory footprint of \name is $2\Psi$ bytes for a model with $\Psi$ parameters, given enough data parallelism. On a cluster of V100 GPUs with 32GB of memory, this allows us to fit about a 14B parameter model without any model parallelism after accounting for 2GB in constant buffers. This is beyond the size of any model that we have seen in literature. Furthermore, on a HPC cluster composed of systems like the DGX-2 box, \name allows us to fit a model with over $200B$ parameters using model parallelism such as tensor slicing or model pipelining. Training such a model would require near exa-flop scale supercomputers with tens of thousands of V100 like GPUs, requiring next generation of supercomputers. However, if one were to look into the future, where tens of thousands of DGX-2 boxes were connected by infiniband like interconnect, it is interesting to ponder, if and how we could train a model with a trillion parameters. Here, we build the final piece of technology that will enable training  such a model with good efficiency, when the massively powerful hardware required to train such a model does become ready.

Note that with 14B parameters per GPU, it is possible to trivially get to a trillion parameter model by using 72 way model parallelism across multiple DGX-2 boxes. However, crossing a single DGX-2 box boundary with model parallelism greatly reduces the available inter process communication bandwidth, from near 300 GB/s between GPUs, to a meager 12.5 GB/s across GPUs. At such communication bandwidth, model parallelism will simply not scale. Therefore, it is critical that the entire model fits within a single node such as a DGX-2 box.
\end{comment}


==> unprecedented_scale.tex <==
\subsection{Unprecedented Scale}
Unprecedented Model Scale: 

ZeRO-Infinity offers a multi-generational leap in DL training system technology offering a path to supporting the next 1000x increase in model-scale by efficiently exploiting the heterogeneous memory systems on current and future generation of hardware. It can train a model with over a trillion parameters on a single NVIDIA DGX-2 box, and with a few dozen of these in a cluster, ZeRO-Infinity can train models with tens of trillion parameters (see Figure X for details).

To enable model training at this scale, ZeRO-Infinity is comprised of four major technologies that work together to target different memory bottlenecks for training: 

1.	ZeRO Stage 3 for removing all memory redundancies in data parallel training by partitioning model states across data parallel processes, 
2.	ZeRO Offload Engine for fully exploiting modern heterogeneous memory architectures by offloading partitioned model states to CPU or NVME device memory, 
3.	Activation checkpointing with CPU offload for reducing activation memory footprint that can become the memory bottleneck on the GPU after the memory required by the model states are addressed by ZeRO Stage3 and the ZeRO Offload Engine, and 
4.	Partially Sequential Execution of Parallel Operators, a computation rescheduling technique that works together with ZeRO Stage 3 to reduce memory footprint of incredibly massive individual layers that can be too large to fit in GPU memory even one layer at a time.

Learn more on these four technologies. (folded)

ZeRO Stage 3: The first piece in ZeRO-Infinity is the ZeRO Stage 3 that fully addresses the memory redundancy of data parallel training. As discussed above, ZeRO-3 supports partitioning all three model states: parameters, gradients, and optimizer states across all data parallel process, allowing the model states to be fully partitioned among the data parallel processes. By leveraging ZeRO-Stage 3, ZeRO Infinity can exploit the aggregate GPU memory available on a cluster to fit the model states. ZeRO Stage 3 can support a trillion parameters with 1024 NVIDIA V100 GPUs (see Table 1 for details).

ZeRO Offload Engine: State of art DL training systems such as 3D parallelism is bottlenecked by the aggregate GPU memory. However, modern GPU clusters have 2-3x more total CPU memory than total GPU memory, and a whopping, 10-20x more total NVMe memory (see Table 2 for details). Furthermore, the state-of-art NVMe technology allows for over 25GB/s of achievable read/write speeds even at these massive sizes, comparable to PCI-E Gen 4 links. While this is nowhere close to the peak GPU memory bandwidth (1TB/s), we realized that though careful design and optimizations we can fully exploit these memories to achieve extreme model scales without being bottlenecked by their bandwidth. 

The new NVMe Offload Engine is the brainchild of this realization. It is a novel data transfer library consisting of carefully crafted high performance data movement kernels for training DL models. It can fully exploit both the CPU memory and the NVMe memory to offload the model states partitioned by ZeRO Stage-3, allowing ZeRO-Infinity to create and train models at an unprecedented scale. ZeRO-Infinity can train a whopping trillion parameter model on a single GPU of a NVIDIA V100 DGX-2 node (100x larger than the current state-of-art for single GPU), or it can train models with over 20 trillion parameters on 16 such nodes (50x larger than 3D parallelism on the same number of nodes). See Table 1 for details  

Activation checkpointing with CPU offload:  Models with over ten billion parameters require significant amount of memory for storing activations (see Table 3 for details), beyond what is available on a single GPU. To avoid running out of memory, we can use activation checkpointing, where instead of storing all activations, we only store them at specified intervals to save memory at the expense of activation re-computation in the backward pass. Activation checkpointing can reduce the activation memory footprint by orders of magnitude, however, for multi-trillion parameter model, the memory requirement post activation checkpointing is still too large to fit in GPU memory. To address this, we support activation checkpointing with CPU offload, allowing all the activation to reside in CPU. 

Partially Sequential execution of parallel operations: Models with hundreds of billions to trillions of parameters require significant memory even for individual layers. As a example, a single intermediate layer in a transformer model with with a hidden dimension of 64K requires over 64 GB of memory to store the parameter and gradients in fp16. Computing the forward and backward on such a layer not just requires over 64GB of working memory, but also at least two contiguous memory buffers of over 32GB, one for parameter and another for the gradients, which is simply not possible even on NVIDIA 80GB A100 cards due to general memory fragmentation. 

Model parallelism solves this issue by partitioning the individual layer across GPUs. Alternatively, it is possible to partition this layer in the same way as with model parallelism, but execute these partitions in sequence on the same GPU. We call this approach partially sequential execution of parallel operators. When combined with ZeRO Stage 3, this reduces the working memory proportional to the number of partitions, supporting arbitrarily large hidden sizes which would otherwise require model parallelism to fit even a single model layer. 

==> where-did-memory-go.tex <==
\section{Where Did All the Memory Go?}
Let's take a step back to examine the memory consumption of the current training system.  For example,  a 1.5B parameter GPT-2 model requires 3GB of memory for its weights (or parameters) in 16-bit precision, yet, it cannot be trained on a single GPU with 32GB memory using Tensorflow or PyTorch.  One may wonder where all the memory goes.
During model training, most of the memory is consumed by {\it model states}, i.e., tensors comprising of optimizer states, gradients, and parameters. Besides these model states, the rest of the memory is consumed by activations, temporary buffers and fragmented memory which we call \emph{residual states}. We look at the memory consumption from both in details.
\begin{comment}
and iii) temporary buffers. It is possible to trivially  Here we look at the memory consumed by latter two of the three.
\end{comment}

\subsection{Model States: Optimizer States, Gradients and Parameters} The majority of the device memory is consumed by model states during training.  Consider for instance, Adam~\cite{DBLP:journals/corr/Adam}, one of the most popular optimizers for DL training. Adam requires storing two optimizer states, i) the time averaged momentum and ii) variance of the gradients to compute the updates. Therefore, to train a model with ADAM, there has to be enough memory to hold a copy of both the momentum and variance of the gradients. In addition, there needs to be enough memory to store the gradients and the weights themselves. Of these three types of the parameter-related tensors, the optimizer states usually consume the most memory, specially when mixed-precision training is applied.

\textbf{Mixed-Precision Training} The state-of-the-art approach to train large models on the current generation of NVIDIA GPUs is via mixed precision (fp16/32) training~\cite{micikevicius2017mixed}, where parameters and activations are stored as fp16, enabling the use of the high throughput tensor core units~\cite{nvidia-volta-arch} on these GPUs. During mixed-precision training, both the forward and backward propagation are performed using fp16 weights and activations. However, to effectively compute and apply the updates at the end of the backward propagation, the mixed-precision optimizer keeps an fp32 copy of the parameters as well as an fp32 copy of all the other optimizer states. 

Let's take Adam as a concrete example.  Mixed precision training of a model with $\Psi$ parameters using Adam requires enough memory to hold an $fp16$ copy of the parameters and the gradients, with memory requirements of $2\Psi$ and $2\Psi$ bytes respectively.  In addition, it needs to hold the optimizer states: an $fp32$ copy of the parameters, momentum and variance, with memory requirements of $4\Psi$, $4\Psi$, and $4\Psi$ bytes, respectively.  Let's use $K$ to denote the memory multiplier of the optimizer states, i.e., the additional memory required to store them is $K\Psi$ bytes. Mixed-precision Adam has $K=12$. In total, this results in $2\Psi + 2\Psi + K\Psi = 16\Psi$ bytes of memory requirement. 
For a model such as GPT-2 with $1.5$ Billion parameters, this leads to a memory requirement of at least $24\,GB$, which is significantly higher than the meager $3\,GB$ of memory required to hold the $fp16$ parameters alone.

\subsection{Residual Memory Consumption}
\textbf{Activations} can take up a significant amount of memory \cite{DBLP:journals/corr/ChenXZG16} during training.  As a concrete example, the 1.5B parameter GPT-2 model trained with sequence length of 1K and batch size of 32 requires about 60\,GB of memory\footnote{The activation memory of a transformer-based model is proportional to the number of transformer layers $\times$ hidden dimensions $\times$  sequence length $\times$ batch size.  For a GPT-2 like architecture the total activations is about  $12 \times hidden\_dim \times batch \times seq\_length \times transformer\_layers$.}.  Activation checkpointing (or activation recomputation) is a common approach to reduce the activation memory by approximately the square root of the total activations at the expense of $33\%$ re-computation overhead \cite{DBLP:journals/corr/ChenXZG16}. This would reduce the activation memory consumption of this model to about 8\,GB.

Despite the significant reduction, the activation memory can grow quite large for bigger models even with activation checkpointing. For example, a GPT-like model with 100 billion parameters requires around 60 GB of memory for batch size 32, even when using activation checkpointing.

\begin{comment}
the amount of activation memory for a transformer based language model is proportional to the batch size, sequence length, hidden dimension and the number of layers . 
Activations take a non-trivial amount of memory even when using techniques such as activation checkpointing which significantly reduce the memory required by the activations at the expense of a $33\%$ re-computation overhead\cite{}.


For example, lets consider the 1.5B parameter GPT-2 model. Without activation checkpointing a transformer model produces $O(\frac{model\_size}{hidden\_dim}*seq\_length*batch$) activation, while with activation checkpointing it produces $O(\frac{model\_size}{hidden\_dim}*seq\_length*batch$) activations if we stored the activations only at the transformer layer boundary. For a batch size of 32, the GPT-2 models will therefore produce about 60GB of activations in fp16, while with activation checkpointing, it produces about 5 GB of activations.
\end{comment}

\textbf{Temporary buffers} used for storing intermediate results consumes non-trivial amount of memory for large models.   Operations such as gradient all-reduce, or gradient norm computation tend to fuse all the gradients into a single flattened buffer before applying the operation in an effort to improve throughput. For example, the bandwidth of all-reduce across devices improves with large message sizes. While the gradient themselves are usually stored as fp16 tensors, the fused buffer can be an fp32 tensor depending on the operation. When the size of the model is large, these temporary buffer sizes are non-trivial. For example, for a model with 1.5B parameters, a flattened fp32 buffer would required $6\,GB$ of memory. 

\textbf{Memory Fragmentation: }  So far we have discussed the actual memory consumption during training. Additionally, it is possible to run out of usable memory even when there is plenty of available memory. This can happen with memory fragmentation. A request for a memory will fail if there isn't enough contiguous memory to satisfy it, even if the total available memory is larger than requested. We observe significant memory fragmentation when training very large models, resulting in out of memory issue with over 30\% of memory still available in some extreme cases.
\begin{comment}

Training a large model with many layers can runs out of memory during training, even when there is plenty of available memory. 

We find that activation checkpointing and backward propagation can cause heavy memory fragmentation, making significant portion of the GPU memory unusable, even when there is plenty of available memory. 
The memory fragmentation is caused by activation checkpointing and backward propagation allocating long term and shot term memory in an interleaved fashion. During the forward propagation, temporary buffers are created in between the creation of each activation checkpoint, causing memory fragmentation. Similarly, in backward propagation working memory is allocated between computation of the gradients, also causing memory fragmentation. We find that for models with hundreds of layers, memory fragmentation can make over 30\% of the GPU memory unusable.
\end{comment}


==> zero-and-model-parallelism.tex <==
\section{\name \& Model Parallelism}\label{sec:modelparallelism}
Since \name solves the memory inefficiency problem of data parallelism, one may wonder: Is model parallelism still needed, and when?  Does \name work with model parallelism and how?  

With \name, model parallelism becomes less essential / attractive for the sole purpose of reducing memory footprint and fitting large models.  \name-powered data paralellism ($P_{os+g+p}$) is at least as effective on reducing per-device memory footprint as model parallelism, and it could be more effective sometimes when model parallelism cannot divide the model evenly. It also has comparable or better scaling efficiency.  Furthermore, data parallelism is so easy to use and it is widely applicable across different workloads, while model parallelism approaches today often need some work from model developers to revise their model, system developers to work out distributed operators, and the existing work like Megatron only supports a limited set of operators and models.

That being said, there are still cases where model parallelism can be helpful: when aggregated batch size of using data parallelism alone is too big to have good convergence.  In those case, model parallelism can be combined with \name-powered data parallelism to fit the model with an acceptable aggregated batch size.

\name (or \name-powered data parallelism) can be combined with any form of model parallelism to train very large models. The total memory saving can be computed as the product of the saving factor from model parallelism and that from \name.  More specifically, if model parallelism of $N_m$ reduces per-device model size from $\Psi$ to $Y$ where $Y = \Psi / N_m$, the total memory consumption per device is given by $\frac{1}{N_m}\times (4\Psi+\frac{12\Psi}{N_d})$, $\frac{1}{N_m}\times (2\Psi+\frac{14\Psi}{N_d})$, and $\frac{16\Psi}{N_d \times N_m}$, using $P_{os}$, $P_{os+g}$ and $P_{os+g+p}$, respectively. As a concrete example, a 32 B parameter with 16-way model parallelism and 64-way data parallelism will consume 8.4GB, 4.4GB and 0.5GB, with $P_{os}$, $P_{os+g}$ and $P_{os+g+p}$ respectively, while without using \name, it would consume at least 32GB of memory per GPU.

With the multiplicative memory saving, combining \name with model parallelism enables the current generation hardware to run significantly larger model with the same model parallelism degree efficiently, without requiring to go across node boundaries. 
Table ~\ref{tab:largest-model} shows an upper bound on the largest model that can be run for a given degree of model parallelism and data parallelism.  In the table the baseline columns represent the existing approach of using data and model parallelism. Note that with 16-way model parallelism, in theory (without any activation and other memory overheads), the baseline can at most run a 32B parameter model, while \name, with its various memory optimizations turned on, can fit 121 Billion, 230 Billion and 2 Trillion using $P_{os}$, $P_{os+g}$, P$_{os+g+p}$, respectively. 

